Speech2Phone: A Novel and Efficient Method for Training Speaker Recognition Models

In this paper we present an efficient method for training models for speaker recognition using small or under-resourced datasets. This method requires less data than other SOTA (State-Of-The-Art) methods, e.g. the Angular Prototypical and GE2E loss functions, while achieving similar results to those methods. This is done using the knowledge of the reconstruction of a phoneme in the speaker's voice. For this purpose, a new dataset was built, composed of 40 male speakers, who read sentences in Portuguese, totaling approximately 3h. We compare the three best architectures trained using our method to select the best one, which is the one with a shallow architecture. Then, we compared this model with the SOTA method for the speaker recognition task: the Fast ResNet-34 trained with approximately 2,000 hours, using the loss functions Angular Prototypical and GE2E. Three experiments were carried out with datasets in different languages. Among these three experiments, our model achieved the second best result in two experiments and the best result in one of them. This highlights the importance of our method, which proved to be a great competitor to SOTA speaker recognition models, with 500x less data and a simpler approach.

==> avaliacao-EACL.tex <==

============================================================================ 
EACL 2021 Reviews for Submission #403
============================================================================ 

Title: XYZ: A new and efficient method for training speaker recognition models
Authors: Edresson Casanova, Arnaldo Candido Junior, Frederico Santos de Oliveira, Christopher Shulby, Lucas Rafael Stefanel Gris, Anderson Soares and Sandra Aluísio
============================================================================
                            META-REVIEW
============================================================================ 

Comments: This paper introduces a new method to train speaker recognition systems for open set speaker verification in particular. The proposed method tries to map any segment of speaker audio to a fixed phoneme (/a/) recorded for the same speaker. The method requires less training data than previous SOTA methods that typically use large amounts of data.

Strengths:
- The proposed method needs less training data for open-set speaker verification
- The proposed method gives better results compared to a SOTA model Fast-ResNet-34 trained on a large >2000hrs of VoxCeleb2 training corpus, but tested on a clean VCTK test set for Angular Prototypical loss.
- The paper tries to use multiple open-set speaker verification evaluations using VCTK and Mozilla Common Voices data.

Weaknesses:
- There is no clarity on the scoring or evaluation strategy for speaker identification expts (1 to 3) and speaker verification experiments (4 to 6). (feito)
- It is not clear how the pair of test segments from VCTK and CV databases are tested against the proposed XYZ method. (feito)
- The details of number of positive and negative examples in the speaker verification test sets created by authors on VCTK and CV DBs is not given. (feito)

- Somewhat weak comparison with state of the art. How does the method depend on audio quality? The evaluation presented in the paper does not address this issue directly, but it seems an issue that may impact performance, especially for small datasets. (normalmente a qualidade do áudio não é avaliada na identificação, porém usamos varios datasets com diferentes qualidades .. ) 
- The recorded data is not publicly available, which makes the added value of that limited. The model have not been tested on larger amount of data. ( trabalho futuro iremos disponibilizar um grande dataset .. )
- It would have been better to test the XYZ method against the a few standard speaker verification evaluation sets for which SOTA results are established such as VoxCeleb1 or NIST SRE evaluations. All the eval sets used in the paper are non-standard and constructed by the authors. So it is difficult to say if the VoxCeleb2 SOTA models designed primarily for open-set speaker verification are performing really poor on other datasets. The main positive results for XYZ method against Fast-ResNet-34 with Angular Prototypical loss is the clean train (XYZ data) vs clean test (VCTK).  ( está explicado no artigo pórque não podemos testar no voxceleb, a ideia de verificação de locutores open set não é gerenalizar para qualquer novos locutores? OS modelos não foram ruins apenas o nosso foi proximo com 500x menos dados ..)
- Overall, there appears to be a lot of promise with the proposed methods. However, the paper clearly needs better organization and clarity. Lot of key information are missing are scattered all over. The paper appears still not ready for publication.

============================================================================
                            REVIEWER #1
============================================================================

What is this paper about, what contributions does it make, what are the strengths and weaknesses, what are the questions for the authors?
---------------------------------------------------------------------------
The paper proposes XYZ, an efficient training method for speaker recognition using minimal resources with only 3 hours of audio data in Portuguese from 40 males speakers. They introduce three types of architecture (Dense, Conv, and Recurrent) using shallow architecture and choosing the best model. Compared to other pre-trained models, they show competitive results, such as Fast ResNet–34 trained with 2000 hours data. 

In general, the idea is quite interesting because they try to distinguish how speakers pronounce sounds, but it is still unclear how they train the model to reconstruct the phoneme. The authors should use more space to describe their methods instead of introducing three different architectures that are not essential. The figures (1, 2, 3) take too much space on the paper. I think one figure is enough to illustrate the model.

On the other hand, there is a significant issue in the collection of the XYZ dataset. The authors need to explain further why they only collect audio data from males speakers.

Strengths:
- The proposed method achieves similar results to large pre-trained models.
- The evaluation is done in multiple languages.

Weaknesses:
- Missing baselines for VCTK. Have you check other papers like [1]?
- Major issue in the experiment setting. The dataset only consists of males speakers. By only collecting males speakers, the model will not be robust. The authors need to clarify this matter. 
- The paper is not well structured and not ready for publication.

Questions:
- How do you split the XYZ dataset? Do you check the distribution of the train and test sets? 
- Can you also show the duration of the XYZ train and test sets (in hours/minutes)? 
- What is the difference between XYZ and Speech2Phone? The authors mention "Speech2Phone" in the experiments and conclusion, but the authors do not introduce it in the text.
- I would recommend the authors to add female voices only too to show the model's robustness on mixed-gender voices. I think adding only males voices would not be convincing.

[1] Transfer Learning from Speaker Verification to Multispeaker Text-To-Speech Synthesis https://arxiv.org/pdf/1806.04558.pdf
---------------------------------------------------------------------------


Typos, Grammar, Style and References
---------------------------------------------------------------------------
- Missing spaces (you should check the spacing to help the readers)
- The auhtor different names for their approaches (XYZ and Speech2Phone). I suggest to use Speech2Phone instead of XYZ. XYZ does not have clear semantic meaning.

Typos:
- Line 435 khz -> kHz (y)
- Line 595 Speaker verification Experiments -> Speaker Verification Experiments (y)
- Line 622, 642 experiment -> Experiment (y)
- Line 664 experiment -> Experiment (y)
- Line 667 experiments -> Experiments ? (for consistency) (y)
- Line 700 Table 5: Results for speaker verification Experiments -> Table 5: Results for speaker verification experiments (either lower case all words or capitalize the first character) (y)
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
- The proposed method achieves similar results to large pre-trained models. 
- The evaluation is done in multiple languages. 
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
- The paper does not compare their proposed method with existing baselines for VCTK
- Issue in the experiment setting. They only use male speakers as consideration. I suggest that the authors also need to take only female speakers and test on mixed-gender speakers if they want to evaluate their proposed method's robustness.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                  Overall Recommendation: 2


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about, what contributions does it make, what are the strengths and weaknesses, what are the questions for the authors?
---------------------------------------------------------------------------
The authors present a method for training speaker recognition models that work with small audio datasets. Among the strengths, they state that the method is suitable for use with low-resource languages (although they use Portuguese, they use a small dataset). Another strength is the comparison with other datasets, allowing for a (partial) contrastive evaluation. Among the weaknesses, one could point that two of the methods appear to overfit on small datasets, defeating the purpose. Another weakness lies in the comparison with other works: although the paper contains evaluation of the proposed methods using other datasets, it does not present the overall recognition results framed against previous work. This is important when proposing a method that works on much smaller datasets. Also a possible weakness: although the proposed methods appear to work with clean recordings, it is not clear how they would behave with other data (from the EER results, it can be assumed that resu!
 lts will suffer).

Miscellaneous aspects: how does language change impact performance?
---------------------------------------------------------------------------


Typos, Grammar, Style and References
---------------------------------------------------------------------------
The paper is, in general, well-written and readable. References are up to date.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
New method for training speaker recognition models with small datasets (may provide a way to bootstrap this task for low-resource languages).
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
Somewhat weak comparison with state of the art. How does the method depend on audio quality? The evaluation presented in the paper does not address this issue directly, but it seems an issue that may impact performance, especially for small datasets.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                  Overall Recommendation: 3


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about, what contributions does it make, what are the strengths and weaknesses, what are the questions for the authors?
---------------------------------------------------------------------------
This paper introduces a new method to train speaker recognition system that require less training data than previous SOTA methods (500 times less training data).They investigated fully connected, fully convolutional and recurring models were explored, where  fully connected worked best in open-set scenarios and fully convolutional worked best on the closed-set scenario. They have also recorded a new data set of 40 speakers of Portuguese. 
The strength is the new method for speaker recognitions that requires less data, that have been evaluated in 6 experiments, where they have tested it using 4 different languages and different datasets. Another strength is that they have recorded a new dataset for speaker recognintion.
A weakness is that the recorded training data is not made publically available. Furthermore, it is not certain that the method will be able to learn from a larger amount of data
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
A new method that has been evaluated against SOTA methods and is shown to require less training data. The authors have recorded a new data set of 40 speakers of Portuguese for speaker  recognition training and avaluation.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
The recorded data is not publicly available, which makes the added value of that limited. The model have not been tested on larger amount of data.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                  Overall Recommendation: 3.5


